High-Dimensional Private Empirical Risk Minimization by Greedy Coordinate Descent

In this paper, we study differentially private empirical risk minimization (DP-ERM). It has been shown that the worst-case utility of DP-ERM reduces polynomially as the dimension increases. This is a major obstacle to privately learning large machine learning models. In high dimension, it is common for some model's parameters to carry more information than others. To exploit this, we propose a differentially private greedy coordinate descent (DP-GCD) algorithm. At each iteration, DP-GCD privately performs a coordinate-wise gradient step along the gradients' (approximately) greatest entry. We show theoretically that DP-GCD can achieve a logarithmic dependence on the dimension for a wide range of problems by naturally exploiting their structural properties (such as quasi-sparse solutions). We illustrate this behavior numerically, both on synthetic and real datasets.

==> preamble.tex <==

\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{xcolor}         %

\usepackage{fancyvrb}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{makecell} %
\usepackage{mathtools}

\usepackage{caption}
\usepackage{duckuments}
\usepackage{xspace}

\usepackage[colorinlistoftodos,textsize=scriptsize]{todonotes}
\setlength{\marginparwidth}{1.8cm}
\setuptodonotes{color=pink}
\usepackage{marginnote}
\usepackage{zref-savepos}


\usepackage{titlesec}
\titleformat*{\subparagraph}{\itshape}
\titlespacing{\subparagraph}{%
  0pt}{%
  0\baselineskip}{%
  0.5em}%
\titlespacing{\paragraph}{%
  0pt}{%
  0\baselineskip}{%
  0.5em}%

\newcount\todocount

\newtheorem{claim}{Claim}


\newcommand*{\sketchproofname}{Sketch of Proof}
\newenvironment{sketchproof}[1][\sketchproofname]{
  \begin{proof}[#1] } {
  \end{proof}
}


\usepackage{aligned-overset}



\theoremstyle{theorem}
\newtheorem{innercustomthm}{Theorem}
\newenvironment{restate-theorem}[1]
{\renewcommand\theinnercustomthm{#1}\innercustomthm}
{\endinnercustomthm}

\newcommand{\CDsmooth}{\texttt{CD (smooth clip)}}%
\newcommand{\CDunif}{\texttt{CD (unif clip)}}%


\newcommand{\paul}[1]{\todo{\textbf{Paul:} #1}}
\newcommand{\aurelien}[1]{\todo[color=green]{\textbf{Aurelien:} #1}}
\newcommand{\marc}[2][]{\todo[color=red!60,#1]{\textbf{Marc:} #2}}
\newcommand{\jo}[2][]{\todo[color=blue!60,#1]{\textbf{Jo:} #2}}
\newcommand{\jrs}[1]{\textcolor{red}{#1}}
\renewcommand{\paul}[1]{}
\renewcommand{\aurelien}[1]{}
\renewcommand{\marc}[2][]{}
\renewcommand{\jo}[2][]{}
\renewcommand{\jrs}[1]{}




==> sup-add-expe.tex <==
\begin{figure*}[t]
  \captionsetup[subfigure]{justification=centering}
  \centering
  \begin{subfigure}{0.046\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/xlegend.pdf}
    \begin{minipage}{.1cm}
      \vfill
    \end{minipage}
  \end{subfigure}%
  \begin{subfigure}{0.235\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/sparse_lasso_prox.pdf}
    \caption{\texttt{sparse} \\ LASSO \\ ($\lambda=30$)}
    \label{fig:expe-sparse-lasso}
  \end{subfigure}%
  \begin{subfigure}{0.235\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/california_l1_norm_prox.pdf}
    \caption{\texttt{california}\\ LASSO \\  ($\lambda=0.1$)}
    \label{fig:expe-california}
  \end{subfigure}%
  \begin{subfigure}{0.235\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/dorothea_norm_prox.pdf}
    \caption{\texttt{dorothea}\\ Logistic + L1 \\  ($\lambda=0.1$)}
    \label{fig:expe-dexter}
  \end{subfigure}%
  \begin{subfigure}{0.235\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/madelon_l1_norm_prox.pdf}
    \caption{\texttt{madelon}\\ Logistic + L1 \\  ($\lambda=0.05$)}
    \label{fig:expe-madelon-l1}
  \end{subfigure}%

  \caption{Relative error to non-private optimal for DP-CD, DP-GCD and
    DP-SGD on different problems. On the x-axis, $1$ tick represents
    a full access to the data: $p$ iterations of DP-CD, $n$ iterations
    of DP-SGD and $1$ iteration of DP-GCD. Number of iterations,
    clipping thresholds and step sizes are tuned simultaneously for
    each algorithm. We report min/mean/max values over 5~runs.}
  \label{fig:expe-nice}
\end{figure*}



==> sup-lower-bound-extension.tex <==
\section{Lower bounds for Strongly-Convex Functions}
\label{sec:lower-bounds-strongl}






==> sup-proof-utility-bak.tex <==

\section{Proof of Utility}
\label{sec-app:proof-utility}

To prove Theorem~\ref{thm:greedy-cd-utility}, we first prove a technical lemma
(Section~\ref{sec:technical-lemmas})
and a descent lemma (Section~\ref{sec:descent-lemma}). We then use these
results to prove the two
statements of Theorem~\ref{thm:greedy-cd-utility}: the general convex case
(Section~\ref{sec:util-gener-conv}) and the strongly convex case
(Section~\ref{sec:util-strongly-conv}).

\subsection{Technical Lemmas}
\label{sec:technical-lemmas}

The following technical lemma will be usefull in our proofs. We will
use it with $\xi_t = F(w^t) - F^*$ and $\beta$ a value that represents
the noise.


\begin{lemma}
  \label{gcd-utility-proof:technical-lemma}
  Let $\{c_t\}_{t\ge 0}^{t=T}$ and $\{\xi_t\}_{t\ge 0}^{t=T}$ be two
  sequences of positive values that satisfy, for some subset of
  indices $\cG_T\subseteq[T]$,
  \begin{align}
    \label{gcd-utility-proof:technical-lemma:assumption-ineq}
    \begin{cases}
      \xi_{t+1} \le \xi_t - \frac{\xi_t^2}{c_t} + \beta,
      & \text{for } t \in \cG_T \enspace, \\
      \xi_{t+1} \le \xi_t
      & \text{otherwise} \enspace,
    \end{cases}
  \end{align}
  such that if $\xi_{t} \le \xi_0$ then $c_t \le c_0$.  Assume that
  $\beta \le c_0$ and $\xi_0 \ge 2 \sqrt{\beta c_0}$. Then:
  \begin{enumerate}
  \item for all $t>0$, $c_t \le c_0$, and there exists $t^*>0$ such
    that $\xi_{t+1}\le\xi_t$ if $t < t^*$ and
    $\xi_t\le 2\sqrt{\beta c_0}$ if $t \ge t^*$.
  \item for all $t \ge 1$,
    $\displaystyle \xi_t \le \frac{c_0}{\abs{\cG_T \cap [t]}} + 2\sqrt{\beta
      c_0}$\enspace.
  \end{enumerate}
\end{lemma}


\begin{proof}
  1. Assume that for $t\ge 0$,
    $\sqrt{\beta c_0} \le \xi_t \le \xi_0$. Then, if
    $t \not\in \cG_T$, $\xi_{t+1}\le\xi_t$ by definition, and
    otherwise $t \in \cG_T$ so
    \begin{align}
      \xi_{t+1}
      \le \xi_t - \frac{\xi_t^2}{c_t} + \beta
      \le \xi_t - \frac{\sqrt{\beta c_0}^2}{c_0} + \beta
      = \xi_t\enspace,
      \label{dp-gcd:techical-lemma-first-ineq}
    \end{align}
    where the second inequality comes from
    $\xi_t \ge \sqrt{\beta c_0}$ and $\xi_t \le \xi_0$ (which implies
    $c_t \le c_0$). We now define the following value $t^*$, which
    defines the point of rupture between two regimes for $\xi_t$:
    \begin{align}
      t^* = \min \left\{ t \ge 0 \,\middle|\, \xi_t \le \sqrt{\beta c_0} \right\}\enspace.
    \end{align}
    Let $t < t^*$, assume that $\xi_t \le \xi_0$,
    then~\eqref{dp-gcd:techical-lemma-first-ineq} holds, that is
    $\xi_{t+1} \le \xi_t \le \xi_0$. By induction, it follows that for
    all~$t < t^*$, $\xi_{t+1} \le \xi_t \le \xi_0$ and $c_t \le c_0$.

    Remark now that $\xi_{t^*} \le \sqrt{\beta c_0}$, we prove by
    induction that $\xi_t$ stays under $2\sqrt{\beta c_0}$ for
    $t\ge t^*$.  Assume that for some $t \ge t^*$,
    $\xi_t \le 2\sqrt{\beta c_0}$. If $t \not\in\cG_T$,
    $\xi_{t+1}\le\xi_t\le 2\sqrt{\beta c_0}$. Otherwise, there are two
    possibilities. If $\xi_{t} \le \sqrt{\beta c_0}$, then
    \begin{align}
      \xi_{t+1}\le \xi_t - \frac{\xi_t^2}{c_t} + \beta \le \sqrt{\beta
      c_0} + \beta \le 2\sqrt{\beta c_0}\enspace,
    \end{align}
    and $\xi_{t+1} \le 2\sqrt{\beta c_0}$. Otherwise,
    $\sqrt{\beta c_0} \le \xi_t \le 2\sqrt{\beta c_0} \le \xi_0$
    and~\eqref{dp-gcd:techical-lemma-first-ineq} holds, which gives
    $\xi_{t+1} \le \xi_t \le 2\sqrt{\beta c_0}$. We proved that for
    $t \ge t^*$, $\xi_t \le 2\sqrt{\beta c_0}$, which
    concludes the proof of the first part of the lemma.

    2. We start by proving this statement for $0 < t < t^*-1$. Define
    $\omega = \frac{2u}{c_0}$ and $u = \sqrt{\beta c_0}$. If
    $t \not\in \cG_T$, $\xi_{t+1}\le\xi_t$. Otherwise, the assumption
    on $\xi_t$ implies, by the first part of the lemma,
    $\xi_{t+1} \le \xi_t - \frac{\xi_t^2}{c_t} + \beta \le \xi_t -
    \frac{\xi_t^2}{c_0} + \beta$, which can be rewritten
    \begin{align}
      \xi_{t+1} - u \le (1 - \omega) (\xi_t - u) - \frac{(\xi_t - u)^2}{c_0} \enspace,
      \label{dp-gcd:techical-lemma-nice-recursion}
    \end{align}
    since
    $(1 - \omega) (\xi_t - u) - \frac{(\xi_t - u)^2}{c_0} = \xi_t -
    \omega \xi_t - u + \omega u - \frac{\xi_t^2}{c_0} - \frac{2\xi_t
      u}{c_0} - \frac{u^2}{c_0} = \xi_t - \frac{\xi_t^2}{c_0} - u +
    \omega u - \frac{u^2}{c_0}$, and
    $\omega u - \frac{u^2}{c_0} = \frac{u^2}{c_0} = \beta$. Since
    $t < t^*-1$, $\xi_{t+1} - u > 0$ and $\xi_t - u > 0$, we can thus
    divide ~\eqref{dp-gcd:techical-lemma-nice-recursion} by
    $(\xi_{t+1} - u)(\xi_{t} - u)$ to obtain (when $t \in \cG_T$):
    \begin{align}
      \frac{1}{\xi_t - u}
      \le \frac{1 - \omega}{\xi_{t+1} - u} - \frac{\xi_t - u}{(\xi_{t+1} - u) c_0}
      \le \frac{1 - \omega}{\xi_{t+1} - u} - \frac{1}{c_0}
      \le \frac{1}{\xi_{t+1} - u} - \frac{1}{c_0}\enspace,
    \end{align}
    where the second inequality comes from
    $\xi_{t+1} - u \le \xi_t - u$ from the first part of the lemma. By
    applying this inequality (as well as $\xi_{t+1}\le\xi_t$ for
    $t\not\in\cG_t$) recursively and taking the inverse of the result,
    we obtain the desired inequality
    \begin{align}
      \xi_t \le \frac{c_0}{\abs{\cG_T \cap [t]}} + \sqrt{\beta c_0} \le
      \frac{c_0}{\abs{\cG_T \cap [t]}} + 2\sqrt{\beta c_0}
      \enspace,
    \end{align}
    for all $0 < t < t^*$.

    For $t \ge t^*$, we have already proved that
    $\xi_t \le 2\sqrt{\beta c_0} \le \frac{c_0}{\abs{\cG_T \cap [t]}}
    + 2\sqrt{\beta c_0}$, which concludes our proof.
\end{proof}


\begin{lemma}
  \label{gcd-utility-proof:sum-square-lemma}
  Let $a, b \in \RR$, then $\abs{a+b}^2 \le 2\abs{a}^2 + 2\abs{b}^2$
  and thus
  \begin{align}
    - \abs{a}^2 \le - \frac{1}{2} \abs{a+b}^2 + \abs{b}^2\enspace.
  \end{align}
\end{lemma}
\begin{proof}
  The first inequality comes from
  \begin{align}
    \abs{a+b}^2 - 2\abs{a}^2 - 2\abs{b}^2
    = - \abs{a}^2 + 2ab - \abs{b}^2
    = - (a - b)^2
    \le 0\enspace,
  \end{align}
  Subtracting $2\abs{a}^2 + \abs{a+b}^2$ to each side and dividing by
  $2$ then yields the result.
\end{proof}

\begin{lemma}[From lemma 1 in \cite{karimireddy2019Efficient}]
  \label{gcd-utility-proof:correspondance-gs-s-with-s}
  Let $f: \RR^p \rightarrow \RR$ be a differentiable function,
  $\lambda > 0$, and $w \in\RR$. We define
  \begin{align}
    s_j^b(w) =
    \begin{cases}
      0 & \text{if } w_j = 0 \textnormal{ and } \abs{\nabla_j f(w) + b_j} \le \lambda \\
      \nabla_j f(w) + b_j - \lambda & \textnormal{if } w_j = 0 \textnormal{ and } \nabla_j f(w) + b_j \ge \lambda \\
      \nabla_j f(w) + b_j + \lambda & \textnormal{if } w_j = 0 \textnormal{ and } \nabla_j f(w) + b_j \le -\lambda \\
      \nabla_j f(w) + b_j + \sign(w_j) \lambda & \textnormal{otherwise}
                                           \enspace.
    \end{cases}
  \end{align}
  Then, for $M_1, \dots, M_p > 0$,
  \begin{align}
    \argmax_{j\in[p]}
    \min_{s\in\partial\psi_j(w_j)} \frac{1}{\sqrt{M_j}} \absbig{\nabla_j f(w) + b_j + s}
    = \argmax_{j\in[p]} \frac{1}{\sqrt{M_j}} \absbig{s_j^b(w)}
    \enspace.
  \end{align}
\end{lemma}

\begin{proof}
  Take $j \in [p]$. If $w_j \neq 0$, then
  $\partial \psi_j(w_j) = \lambda \sign(w_j)$. This gives
  \begin{align}
    \min_{s\in\partial\psi_j(w_j)} \frac{1}{\sqrt{M_j}} \absbig{\nabla_j f(w) + b_j + s}
    & = \frac{1}{\sqrt{M_j}} \absbig{\nabla_j f(w) + b_j + \lambda \sign(w_j)}
      \enspace.
  \end{align}
  And if $w_j = 0$, then
  $\partial \psi_j(w_j) = [-\lambda, +\lambda]$, and it holds that
  \begin{align}
    \min_{s\in\partial\psi_j(w_j)} \frac{1}{\sqrt{M_j}} \absbig{\nabla_j f(w) + b_j + s}
    & = \begin{cases}
          0 & \textnormal{if } \abs{\nabla_j f(w) + b_j} \le \lambda  \\
          \frac{1}{\sqrt{M_j}} \nabla_j f(w) + b_j - \lambda & \textnormal{if } \nabla_j f(w) + b_j \ge \lambda  \\
          \frac{1}{\sqrt{M_j}} \nabla_j f(w) + b_j + \lambda & \textnormal{if } \nabla_j f(w) + b_j \le - \lambda  \\
        \end{cases}
      \enspace.
  \end{align}
  All put together,
  $\min_{s\in\partial\psi_j(w_j)} \frac{1}{\sqrt{M_j}}
  \absbig{\nabla_j f(w) + b_j + s}$ evaluates to
  $\frac{1}{\sqrt{M_j}} s_j^b(w)$, which is the result of the lemma.
\end{proof}

\subsection{Descent Lemma}
\label{sec:descent-lemma}

\subsubsection{Progress in \good steps}
\label{sec:progress-good-steps}


\begin{lemma}
  Let $T > 0$. Let $\{ w^t \}_{t=0}^{t=T}$ be the iterates,
  $\{ j_t \}_{t=0}^{t=T}$ the coordinates chosen by the noisy \GSs and
  $\{ j^*_t \}_t$ the exact \GSs coordinates for
  \Cref{algo:private-greedy-coordinate-descent} with noise scales
  $\sigma_j \le \sigma_{\max}$. Let $t \in \cG_T$ be a \good step. The
  following inequality holds
  \label{gcd-utility-proof:good-step-descent-lemma}
  \begin{align}
    F(w^{t+1}) - F(w^t)
    & \le
      - \frac{1}{2M_j} s_j(w^t)^2
      + \frac{1}{2M_j} \abs{\eta_{j}^t}^2
      \enspace.
  \end{align}
\end{lemma}

\begin{proof}
  In this proof, we use the notations $\psi(w) = \lambda \norm{w}_1$
  and $\psi_j(w_j) = \lambda \abs{w_j}$.  Since $\psi$ is separable,
  $F(w^{t+1})$ can be decomposed as
  \begin{align}
    F(w^{t+1})
    & = f(w^{t+1})
      + \psi(w^{t+1})
      = f(w^{t+1})
      + \psi(w^{t})
      + \psi_{j_t}(w_{j_t}^{t+1})
      - \psi_{j_t}(w_{j_t}^{t})
      \enspace.
      \label{gcd-utility-proof:descent-lemma:F-as-sum}
  \end{align}

  As $t \in \cG_T$ is a \good step, optimality condition of the
  proximal operator gives a real number
  $\xi_j \in \partial \psi_j(w^{t+1}_j)$ such that
  $w^{t+1} = w^t - \frac{1}{M_j} ( \nabla_j f(w^t) + \xi_j + \eta_j)$.
  Smoothness of $f$ then implies
  \begin{align}
    f(w^{t+1})
    & \le
      f(w^t)
      + \scalar{\nabla f(w^t)}{w^{t+1} - w^t}
      + \frac{1}{2} \norm{w^{t+1}-w^t}_{M}^2 \nnl
    & =
      f(w^t)
      - \frac{1}{M_{j_t}} \nabla_jf(w^t) (
      \nabla_j f(w^t) + \xi_j + \eta_j)
      + \frac{1}{2M_j} (\nabla_j f(w^t) + \xi_j + \eta_j)^2 \nnl
    & =
      f(w^t)
      - \frac{1}{M_{j_t}} \nabla_jf(w^t)
      (\nabla_j f(w^t) + \xi_j)
      - \frac{1}{M_{j_t}} \nabla_jf(w^t) \eta_j \nnlq
      + \frac{1}{2M_j} (\nabla_j f(w^t) + \xi_j)^2
      + \frac{1}{M_j} (\nabla_j f(w^t) + \xi_j) \eta_j
      + \frac{1}{2M_j} \eta_j^2 \nnl
    & =
      f(w^t)
      - \frac{1}{2M_j} (\nabla_j f(w^t) + \xi_j)^2
      + \frac{1}{M_{j_t}} \xi_j
      (\nabla_j f(w^t) + \xi_j + \eta_j)
      + \frac{1}{2M_j} \eta_j^2
      \enspace.
      \label{gcd-utility-proof:descent-lemma:smoothness-upper-bound}
  \end{align}
  Since $\xi_j \in \partial \psi_j(w^{t+1}_j)$, the subdifferential of
  $\psi_j$ at $w^{t+1}_j$, it holds that
  \begin{align}
    \psi_{j_t}(w_{j_t}^{t+1}) - \psi_{j_t}(w_{j_t}^{t})
    \le \xi_j(w_{j_t}^{t+1}-w_{j_t}^t)
    = - \frac{1}{M_j} \xi_j(\nabla_j f(w^t) + \xi_j + \eta_j)\enspace.
    \label{gcd-utility-proof:descent-lemma:reg-convexity-upper-bound}
  \end{align}
  We now
  plug~\eqref{gcd-utility-proof:descent-lemma:smoothness-upper-bound}
  and~\eqref{gcd-utility-proof:descent-lemma:reg-convexity-upper-bound}
  in~\eqref{gcd-utility-proof:descent-lemma:F-as-sum} to obtain
  \begin{align}
    F(w^{t+1})
    & \le F(w^{t})
      - \frac{1}{2M_j} (\nabla_j f(w^t) + \xi_j)^2
      + \frac{1}{2M_j} \abs{\eta_j}^2\enspace.
  \end{align}
  At this point, we use the fact that $t$ is a \good step, and
  distinguish two cases. First, assume that $t$ is a \good step with
  $w_j^t \neq 0$. Then $w_j^{t}$ and $w_j^{t+1}$ have the same sign
  and are non-zero. Thus
  $\xi=\sign(w_j^{t+1})\lambda=\sign(w_j^t)\lambda$, which we can
  replace in
  $- \frac{1}{2M_j} (\nabla_j f(w^t) + \xi_j)^2 = - \frac{1}{2M_j}
  (\nabla_j f(w^t) + \sign(w_j^t)\lambda)^2 = - \frac{1}{2M_j} s_j(w^t)^2$.

  Second, assume that $t$ is a \good step with $w_j^t = 0$. We have
  $w_j^{t+1}\neq 0$, otherwise the step would be \bad. This in turns
  implies that $\abs{\nabla_j f(w^t)}\ge\lambda$. Then either
  $\nabla_j f(w^t) \le -\lambda$ (in which case $w_j^{t+1}>0$ and
  $\xi_j=\lambda$) and we obtain
  $- \frac{1}{2M_j} (\nabla_j f(w^t) + \xi_j)^2 = - \frac{1}{2M_j}
  (\nabla_j f(w^t) + \lambda)^2 = - \frac{1}{2M_j} s_j(w^t)^2$. Either
  $\nabla_j f(w^t) \ge \lambda$, and the same argument gives
  $- \frac{1}{2M_j} (\nabla_j f(w^t) + \xi_j)^2 = - \frac{1}{2M_j}
  (\nabla_j f(w^t) - \lambda)^2 = - \frac{1}{2M_j} s_j(w^t)^2$.

  Thus, in any \good step, we have
  \begin{align}
    F(w^{t+1})
    & \le F(w^{t})
      - \frac{1}{2M_j} s_j(w^t)^2
      + \frac{1}{2M_j} \abs{\eta_j}^2
      \enspace,
  \end{align}
  which is the desired result.
\end{proof}







\begin{lemma}
  \label{gcd-utility-proof:quantify-update-lemma}
  Let $f : \RR^p\rightarrow\RR$ a differentiable function,
  $\lambda\ge 0$ and $\xi\in[-\lambda,\lambda]^p$ and $w \in \RR^p$,
  then
  \begin{align}
    - \frac{1}{M_{j^*}} s_{j^*}(w)^2
    & = \min_{h\in\RR^p} \left\{\scalar{\nabla f(w^t)}{h}
      + \frac{1}{2}\norm{h}_{M^{-1},1}^2
      + \lambda\norm{w^t + h}_1 - \lambda\norm{w^t}_1
      \right\}
      \enspace.
  \end{align}
\end{lemma}

\begin{proof}
  By a careful examination of the minimum, we have
  \begin{align}
    - \frac{1}{M_{j^*}} s_{j^*}(w)^2
    & = \min_{h\in\RR^p} \left\{\scalar{s(w)}{h}
      + \frac{1}{2}\norm{h}_{M^{-1},1}^2\right\}
      \enspace.
  \end{align}
  To account for the $\ell_1$-norm regularizer, we remark that for all
  $\xi\in[-\lambda,\lambda]^p$ and $x\in\RR$,
  $\lambda \norm{x}_1 \ge \scalar{\xi}{x}$. Thus, it holds
  that
  \begin{align}
    \lambda \norm{w+h}_1 - \lambda \norm{w}_1
    & \ge \scalar{\xi}{w+h} - \lambda \norm{w}_1
      = \scalar{\xi}{h} + \scalar{\xi}{w} - \lambda \norm{w}_1
      \enspace.
  \end{align}

  The crucial remark is now that we can choose
  $\xi = s(w) - \nabla f(w) \in [-\lambda, \lambda]^p$. Then, for
  $j\in[p]$, we consider two cases. First, if $w_j=0$, then
  $\xi_j w_j - \lambda \abs{w_j} = (\xi_j - \lambda )w_j = 0$. Second,
  if $w_j \neq 0$, then
  $\xi_j w_j - \lambda\abs{w_j} = (s_j(w) - \nabla_j f(w)) w_j -
  \lambda \abs{w_j} = \lambda (\sign(w_j) w_j - \abs{w_j}) = 0$. In
  both cases, we have the inequality
  \begin{align}
    \scalar{s(w)}{h}
    & = \scalar{\nabla f(w)}{h} + \scalar{\xi}{h}
      \le \lambda \norm{w+h} - \lambda \norm{w}
      \enspace.
  \end{align}
  Replacing in the above inequality gives the result of the lemma.
\end{proof}


We now proof our key descent lemma, that will be crucial, with the
above technical lemma, in proving our convergence results. To keep the
notations lighter, we generally omit the $t$ in $j_t$ when it is clear
from the context.

\begin{lemma}
  Let $T > 0$. Let $\{ w^t \}_{t=0}^{t=T}$ be the iterates,
  $\{ j_t \}_{t=0}^{t=T}$ the coordinates chosen by the noisy \GSs and
  $\{ j^*_t \}_t$ the exact \GSs coordinates for
  \Cref{algo:private-greedy-coordinate-descent} with noise scales
  $\sigma_j \le \sigma_{\max}$. Let $t \in \cG_T$ be a \good step. The
  following inequality holds
  \label{gcd-utility-proof:descent-lemma}
  \begin{align}
    F(w^{t+1}) - F(w^*)
    & \le F(w^t) - F(w^*)
      - \frac{(F(w^t) - F(w^*))^2}{16 \norm{w^t-w^*}_{M,1}^2}
      + \frac{\abs{\eta_{j}^t}^2}{2M_{j}}
      + \frac{\abs{\chi_{j}^t}^2}{2M_{j}}
      + \frac{\abs{\chi_{j^*}^t}^2}{4M_{j^*}}
      \enspace.
  \end{align}
\end{lemma}

\begin{proof}
  By \Cref{gcd-utility-proof:good-step-descent-lemma}, since $t$ is a
  \good step, we have
  \begin{align}
    F(w^{t+1}) - F(w^*)
    & \le F(w^t) - F(w^*)
      - \frac{1}{2M_j} s_j^0(w^t)^2
      + \frac{\abs{\eta_{j}^t}^2}{2M_{j}}
      \enspace.
  \end{align}
  This implies that, with \Cref{gcd-utility-proof:sum-square-lemma},
  \begin{align}
    F(w^{t+1}) - F(w^*)
    & \le F(w^t) - F(w^*)
      - \frac{1}{4M_j} s_j^{\chi^t}(w^t)^2
      + \frac{\abs{\chi_{j}^t}^2}{2M_{j}}
      + \frac{\abs{\eta_{j}^t}^2}{2M_{j}}
      \enspace.
  \end{align}
  The noisy \GSs rule, combined with
  \Cref{gcd-utility-proof:correspondance-gs-s-with-s}, then gives
  \paul{todo: is this true that $s_j^b \le s_j^0 + b$ ???}
  \begin{align}
    F(w^{t+1}) - F(w^*)
    & \le F(w^t) - F(w^*)
      - \frac{1}{4M_{j^*}} s_{j^*}^{\chi^t}(w^t)^2
      + \frac{\abs{\chi_{j}^t}^2}{2M_{j}}
      + \frac{\abs{\eta_{j}^t}^2}{2M_{j}} \\
    & \le F(w^t) - F(w^*)
      - \frac{1}{8M_{j^*}} s_{j^*}(w^t)^2
      + \frac{\abs{\chi_{j^*}^t}^2}{4M_{j^*}}
      + \frac{\abs{\chi_{j}^t}^2}{2M_{j}}
      + \frac{\abs{\eta_{j}^t}^2}{2M_{j}}
      \enspace.
  \end{align}
  At this point, we use \Cref{gcd-utility-proof:quantify-update-lemma}
  to obtain the result
  \begin{align}
    \label{gcd-utility-proof:descent-lemma:minim-upper-bound}
    F(w^{t+1})
    & \le F(w^t)
      - \frac{1}{8} \min_{h\in\RR^p} \left\{\scalar{\nabla f(w^t)}{h}
      + \frac{1}{2}\norm{h}_{M^{-1},1}^2
      + \lambda\norm{w^t + h}_1 - \lambda\norm{w^t}_1\right\} \nnlq
      + \frac{\abs{\chi_{j^*}^t}^2}{4M_{j^*}}
      + \frac{\abs{\chi_{j}^t}^2}{2M_{j}}
      + \frac{\abs{\eta_{j}^t}^2}{2M_{j}}
      \enspace.
  \end{align}
  Finally, take $h = - \alpha (w^t - w^*)$ for $\alpha\in\RR$, then by
  convexity of $\psi$,
  \begin{align}
    & \min_{h\in\RR^p} \left\{\scalar{\nabla f(w^t)}{h}
      + \frac{1}{2}\norm{h}_{M^{-1},1}^2
      + \psi(w^t + h) - \psi(w^t)
      \right\} \\
    & \le \min_{\alpha\in\RR} \left\{-\alpha\scalar{\nabla f(w^t)}{w^t - w^*}
      + \frac{\alpha^2}{2}\norm{w^t - w^*}_{M^{-1},1}^2
      + \psi((1-\alpha)w^t + \alpha w^*) - \psi(w^t)
      \right\} \\
    & \le
      \min_{\alpha\in\RR} \left\{-\alpha\scalar{\nabla f(w^t)}{w^t - w^*}
      + \frac{\alpha^2}{2}\norm{w^t - w^*}_{M^{-1},1}^2
      -\alpha(\psi(w^t) - \phi(w^*))
      \right\}
      \enspace.
  \end{align}
  And convexity of $f$ gives
  $- \scalar{\nabla f(w^t)}{w^t - w^*} \le -(f(w^t) - f(w^*))$ thus
  \begin{align}
    & \min_{h\in\RR^p} \left\{\scalar{\nabla f(w^t)}{h}
      + \frac{1}{2}\norm{h}_{M^{-1},1}^2
      + \psi(w^t + h) - \psi(w^t)
      \right\} \\
    & \le \min_{\alpha\in\RR} \left\{-\alpha (F(w^t) - F(w^*))
      + \frac{\alpha^2}{2}\norm{w^t - w^*}_{M^{-1},1}^2
      \right\} \\
    & = - \frac{(F(w^t) - F(w^*))^2}{2\norm{w^t - w^*}_{M^{-1},1}^2}
      \enspace.
  \end{align}
  Plug this back
  in~\eqref{gcd-utility-proof:descent-lemma:minim-upper-bound} and
  subtract $F(w^*)$ on both sides to get the lemma.
\end{proof}


\subsubsection{Controlling \bad steps}
\label{sec:descent-bad-steps}



\begin{lemma}
Let $T > 0$. Let $\{ w^t \}_{t=0}^{t=T}$ be the iterates,
  $\{ j_t \}_{t=0}^{t=T}$ the coordinates chosen by the noisy \GSs and
  $\{ j^*_t \}_t$ the exact \GSs coordinates for
  \Cref{algo:private-greedy-coordinate-descent} with noise scales
  $\sigma_j \le \sigma_{\max}$. Let $t \not\in \cG_T$ be a \bad step. The
  following inequality holds
  \label{gcd-utility-proof:descent-lemma}
  \begin{align}
    F(w^{t+1}) - F(w^*)
    & \le F(w^t) - F(w^*) + \frac{2}{M_j} (\eta_j^t)^2
      \enspace.
  \end{align}
\end{lemma}

\begin{proof}
  The \bad steps can be of two kind: for the chosen coordinate
  $j \in [p]$, either $w_j^t>0$ or $w_j^t < 0$. When $w_j^t > 0$,
  since the step is \bad, it holds that
  $w_j^t - \frac{1}{M_j} (\nabla_j f(w^t) + \lambda + \eta_j^t) < 0$
  and $w_j^{t+1} = 0$. Then the following holds
  \begin{align}
    F(w^{t+1})
    & = f(w^{t+1})
      + \lambda \norm{w^{t+1}}_1 \\
    & \le f(w^{t})
      + \lambda \norm{w^t}_1
      - \nabla_j f(w^t) w_j^t
      + \frac{M_j}{2} \abs{w_j^t}^2
      - \lambda \abs{w_j^t} \\
    & \le F(w^{t})
      - \nabla_j f(w^t) w_j^t
      + \frac{M_j}{2} \abs{w_j^t}^2
      - \lambda w_j^t
      \enspace.
  \end{align}
  We will now use the fact that the step is \bad
  \begin{align}
    F(w^{t+1})
    & \le F(w^{t})
      + M_j w_j^t (
      w_j^t
      - \frac{1}{M_j}
      (\nabla_j f(w^t) + \lambda)) \\
    & = F(w^{t})
      + M_j w_j^t (
      w_j^t
      - \frac{1}{M_j}
      (\nabla_j f(w^t) + \lambda + \eta_j^t)
      - \frac{1}{2} w_j^t
      + \frac{1}{M_j} \eta_j^t) \\
    & = F(w^{t})
      + M_j w_j^t (
      w_j^t
      - \frac{1}{M_j}
      (\nabla_j f(w^t) + \lambda + \eta_j^t))
      - \frac{M_j}{2} (w_j^t)^2
      +  \eta_j^t w_j^t
      \enspace.
  \end{align}
  There, either $\frac{M_j}{2} w_j^t \ge \eta_j^t$ and
  $- \frac{M_j}{2} (w_j^t)^2 + \eta_j^t w_j^t \le 0 \le \frac{2}{M_j}
  (\eta_j^t)^2$, either $\frac{M_j}{2} w_j^t \le \eta_j^t$ and we have
  $- \frac{M_j}{2} (w_j^t)^2 + \eta_j^t w_j^t \le \frac{2}{M_j}
  (\eta_j^t)^2$. Since it was a \bad step, we have
  \begin{align}
    F(w^{t+1})
    & \le F(w^{t})
      + M_j w_j^t (
      w_j^t
      - \frac{1}{M_j}
      (\nabla_j f(w^t) + \lambda + \eta_j^t))
      - \frac{M_j}{2} (w_j^t)^2
      +  \eta_j^t w_j^t \\
    & \le F(w^{t})
      + \frac{2}{M_j} (\eta_j^t)^2
      \enspace,
  \end{align}
  which gives the result after subtracting $F(w^*)$ on both sides.
\end{proof}

\subsection{Counting \good and \bad steps}
\label{sec:counting-good-bad}

\begin{lemma}

\end{lemma}

\begin{proof}
  For $j \in [p]$, we define $S_j \subseteq [T]$ the steps where
  parameter $j$ was updated. Let $t \in S_j$. If $w_j^t = 0$, then either
\end{proof}






\subsection{Utility for General Convex Functions}
\label{sec:util-gener-conv}

\paul{following results may lack a factor 2 but I keep it as-is until
  I am sure of the proof of the above lemmas.}
\paul{there a factor 2 that is lacking in all this proof}

\begin{lemma}
  \label{gcd-utility-proof:general-convex}
  Let $T > 0$. Let $\{ w^t \}_t$ be the iterates, $\{ j_t \}_t$ the
  chosen coordinates and $\{ j^*_t \}_t$ the exact greedy coordinates
  for \Cref{algo:private-greedy-coordinate-descent} with noise scales
  $\sigma_j \le \sigma_{\max}$. Let $\zeta \in (0, 1)$ and
  $\beta = \frac{4\sigma_{\max}^2}{M_{\min}}
  \log(\frac{2Tp}{\zeta})$. Define
  $R_M = \max_{w\in\RR^p} \min_{w^*\in \cW^*} \left\{
    \norm{w-w^*}_{M,1} \mid f(w) \le f(w^0) \right\}$ and assume that
  $f(w^0) - f(w^*) \ge \sqrt{32R_M^2\beta}$, then
  \begin{align}
    \prob{ f(w^T) - f(w^*) \le \frac{8 R_M^2}{T} + \sqrt{32 R_M^2 \beta} } \ge 1 - \zeta.
  \end{align}
  Furthermore, when
  $\sigma_j^2 \le \sigma_{\max}^2 =
  \frac{8TL_{\max}^2\log(1/\delta)}{n^2\epsilon^2}$ and
  $T = \frac{n^{2/3} \epsilon^{2/3} R_M^{2/3}
    M_{\min}^{1/3}}{2^{7/3}L_{\max}^{2/3} \log(1/\delta)^{1/3}}$, then
  \begin{align}
    \prob{ f(w^T) - f(w^*) \le \frac{2^{16/3} R_M^{4/3} L_{\max}^{2/3} \log(1/\delta)^{1/3}}{n^{2/3} \epsilon^{2/3} M_{\min}^{1/3}}\Big(1 + \log\Big(\frac{n^{2/3} p \epsilon^{2/3} R_M^{2/3}
      M_{\min}^{1/3}}{2^{7/3}L_{\max}^{2/3} \log(1/\delta)^{1/3} \zeta}\Big)^{1/2}\Big)} \ge 1 - \zeta.
  \end{align}
\end{lemma}

\begin{proof}
  Let $\phi_t = f(w^t) - f(w^*)$. We upper bound the following
  probability by the union bound, and the fact that for $t \ge 0$, the
  events $E_j^t: $~``coordinate $j$ is updated at step $t$'' for
  $j \in [p]$ partition the probability space:
  \begin{align}
    \prob{
    \exists t \le T - 1,
    \phi_{t+1} \ge
    \phi_t - \frac{\phi_t^2}{8\norm{w^t-w^*}_{M,1}^2} + \beta }
    \le
    \sum_{t=0}^{T-1} \prob{
    \phi_{t+1} \ge
    \phi_{t} - \frac{\phi_{t}^2}{8\norm{w^t-w^*}_{M,1}^2} + \beta } & \\
    =
    \sum_{t=0}^{T-1} \sum_{j=1}^p \prob{
    \phi_{t+1} \ge
    \phi_{t} - \frac{\phi_{t}^2}{8\norm{w^t-w^*}_{M,1}^2} + \beta~\land~E_j^t } \enspace. &
  \end{align}


  \Cref{gcd-utility-proof:descent-lemma} gives
  $\phi_{t+1} \le \phi_t - \frac{\phi_t^2}{8 \norm{w^t-w^*}_{M,1}^2} +
  \frac{1}{2M_{j}} \abs{\eta_{j}^t}^2 + \frac{1}{2M_{j}}
  \abs{\chi_{j}^t}^2 + \frac{1}{4M_{j^*}} \abs{\chi_{j^*}^t}^2$. We
  thus have the following upper bound:
  \begin{align}
    \prob{
    \exists t \le T - 1,
    \phi_{t+1} \ge
    \phi_t - \frac{\phi_t^2}{8\norm{w^t-w^*}_{M,1}^2} + \beta }
    \le
    \sum_{t=0}^{T-1} \sum_{j=1}^p \prob{
    \tfrac{1}{2M_{j}} \abs{\eta_{j}^t}^2 + \tfrac{1}{2M_{j}}
    \abs{\chi_{j}^t}^2 + \tfrac{1}{4M_{j^*}} \abs{\chi_{j^*}^t}^2 \ge \beta } & \\
    \le
    \sum_{t=0}^{T-1} \sum_{j=1}^p \prob{
    \tfrac{1}{2} \abs{\eta_{j}^t}^2 + \tfrac{1}{2}
    \abs{\chi_{j}^t}^2 + \tfrac{1}{4} \abs{\chi_{j^*}^t}^2
    \ge M_{\min} \beta } \enspace. &
  \end{align}
  By the Chernoff bound we have, for $\alpha = \frac{1}{4 \sigma_{\max}^2}$,
  \begin{align}
    \prob{ \tfrac{1}{2} \abs{\eta_{j}^t}^2 + \tfrac{1}{2}
    \abs{\chi_{j}^t}^2 + \tfrac{1}{4} \abs{\chi_{j^*}^t}^2 \ge M_{\min} \beta }
    & \le e^{-\alpha M_{\min} \beta}
      \expec{}{e^{\tfrac{\alpha}{2} \abs{\eta_{j}^t}^2
      + \tfrac{\alpha}{2} \abs{\chi_{j}^t}^2
      + \tfrac{\alpha}{4} \abs{\chi_{j^*}^t}^2}} \\
    & \le 2 e^{-\alpha M_{\min} \beta}
      = 2 e^{-\frac{M_{\min}}{4\sigma_{\max}^2} \beta} \enspace.
  \end{align}
  We now choose $\beta = \frac{4\sigma_{\max}^2}{M_{\min}} \log(\frac{2Tp}{\zeta})$ to obtain
  \begin{align}
    \prob{
    \exists t \le T - 1,
    \phi_{t+1} \ge
    \phi_t - \frac{\phi_t^2}{8\norm{w^t-w^*}_{M,1}^2} + \beta }
    & \le
    \sum_{t=0}^{T-1} \sum_{j=1}^p \frac{\zeta}{Tp}
    = \zeta \enspace.
  \end{align}

  We can now use our \Cref{gcd-utility-proof:technical-lemma}, with
  \begin{itemize}
  \item $\xi_t = f(w^t) - f(w^*)$,
  \item $c_0=8R_M^2$, and $c_t = 8\norm{w^t-w^*}_{M,1}^2$ for $t > 0$,
  \item
    $\beta = \frac{4\sigma_{\max}^2}{M_{\min}}
    \log(\frac{2Tp}{\zeta})$.
  \end{itemize}
  Indeed, by the definition of $R_M$, it holds that $c_t \le c_0$
  whenever $\xi_t \le \xi_0$ (\ie
  $f(w^t) - f(w^*) \le f(w^0) - f(w^*)$). By assumption we have
  $f(w^0) - f
  (w^*) \ge \sqrt{32R_M^2\beta}$, therefore
  $f(w^0)-f(w^*) \ge 2\sqrt{\beta c_0}$, and $\beta \le c_0$,
  the hypothesis of our technical lemma are satisfied.

  This gives the result, with probability at least $1-\zeta$:
  \begin{align}
    f(w^t) - f(w^0)
    & \le \frac{c_0}{t} + 2\sqrt{\beta c_0}
      = \frac{8R_M^2}{t} + \frac{32 L_{\max} R_M \sqrt{8T \log(1/\delta)} \sqrt{\log(2Tp/\zeta)}}{n \epsilon \sqrt{M_{\min}}} \enspace.
  \end{align}
  For
  $T = \frac{n^{2/3} \epsilon^{2/3} R_M^{2/3}
    M_{\min}^{1/3}}{2^{7/3}L_{\max}^{2/3} \log(1/\delta)^{1/3}}$, this
  gives that, with probability at least $1-\zeta$,
  \begin{align}
    f(w^t) - f(w^0)
    & \le
      \frac{2^{16/3} R_M^{4/3} L_{\max}^{2/3} \log(1/\delta)^{1/3}}{n^{2/3} \epsilon^{2/3} M_{\min}^{1/3}}\Big(1 + \log\Big(\frac{n^{2/3} p \epsilon^{2/3} R_M^{2/3}
      M_{\min}^{1/3}}{2^{7/3}L_{\max}^{2/3} \log(1/\delta)^{1/3} \zeta}\Big)^{1/2}\Big) \enspace.
  \end{align}
\end{proof}


\subsection{Utility for Strongly-Convex Functions}
\label{sec:util-strongly-conv}
\paul{this analysis works but better constants can be obtained by a
  refined analysis that uses strong convexity directly.}

\begin{lemma}
  \label{gcd-utility-proof:strongly-convex}
  Let $T > 0$. Let $\{ w^t \}_t$ be the iterates of
  \Cref{algo:private-greedy-coordinate-descent} with noise scales
  $\sigma_j \le \sigma_{\max}$. Let $\zeta \in (0, 1)$, then
  \begin{align}
    \prob{f(w^T) - f(w^*)
    \le (1 - \frac{\mu_M}{2})^T (f(w^0) - f(w^*))
    + \frac{64 T L_{\max}^2 \log(1/\delta)}{M_{\min} \mu_M n^2 \epsilon^2} \log(\frac{2Tp}{\zeta})
    } \ge 1 - \zeta \enspace.
  \end{align}
  And, with $T = \frac{2}{\mu_M} \log(\frac{M_{\min} \mu_M n^2 \epsilon^2
    (f(w^0)-f(w^*)}{32 L_{\max}^2 \log(1/\delta)})$,
  \begin{align}
    \prob{
    f(w^T) - f(w^*)
    \le
    \frac{64 L_{\max}^2 \log(1/\delta)}{ M_{\min} \mu_M^2 n^2 \epsilon^2}
    \log\Big(\frac{2p}{\mu_M\zeta}\Big)
    \log\Big(\frac{M_{\min} \mu_M n^2\epsilon^2 (f(w^0)-f(w^*)}{32 L_{\max}^2 \log(1/\delta)} \Big)
    } \ge 1 - \zeta \enspace.
  \end{align}
\end{lemma}

\begin{proof}
  When $f$ is $\mu_M$-strongly-convex \wrt the norm
  $\norm{\cdot}_{M,1}$, we have
  \begin{align}
    f(w^t) \ge f(w^*) + \frac{\mu_M}{2}\norm{w^t-w^*}_{M,1}^2,
  \end{align}
  which gives $- \frac{f(w^t) - f(w^*)}{\norm{w^t-w^*}_{M,1}^2} \le - \frac{\mu_M}{2}$.
  We replace this in \Cref{gcd-utility-proof:descent-lemma}, giving
  \begin{align}
    f(w^{t+1}) - f(w^*)
    & \le (1 - \frac{\mu_M}{2}) (f(w^t) - f(w^*))
      + \frac{1}{2M_{j}} \abs{\eta_{j}^t}^2
      + \frac{1}{2M_{j}} \abs{\chi_{j}^t}^2
      + \frac{1}{4M_{j^*}} \abs{\chi_{j^*}^t}^2 \enspace.
  \end{align}
  Analogously to the proof of \Cref{gcd-utility-proof:general-convex},
  we show that
  $\prob{ \exists t \le T - 1, \phi_{t+1} \ge (1 - \frac{\mu_M}{2})
    \phi_t + \beta } \le \zeta$, with
  $\beta = \frac{4\sigma_{\max}^2}{M_{\min}}
  \log(\frac{2Tp}{\zeta})$. This yields that, with probability at
  least $1-\zeta$,
  \begin{align}
    f(w^T) - f(w^*)
    & \le (1 - \frac{\mu_M}{2})^T (f(w^0) - f(w^*))
      + \sum_{t=0}^{T-1}  (1 - \frac{\mu_M}{2})^{T-t} \beta \\
    & \le (1 - \frac{\mu_M}{2})^T (f(w^0) - f(w^*))
      + \frac{2}{\mu_M} \frac{32 T L_{\max}^2 \log(1/\delta)}{M_{\min} n^2 \epsilon^2}
      \log\Big(\frac{2Tp}{\zeta}\Big) \enspace,
  \end{align}
  Additionally, setting
  $T = \frac{2}{\mu_M} \log(\frac{M_{\min} \mu_M n^2 \epsilon^2
    (f(w^0)-f(w^*))}{64 L_{\max}^2 \log(1/\delta) \log(2p/\zeta)})$ gives
  \begin{align}
    \prob{
    f(w^T) - f(w^*)
    \le
    \frac{64 L_{\max}^2 \log(1/\delta) \log(2p/\zeta)}{M_{\min} \mu_M^2 n^2 \epsilon^2
    (f(w^0)-f(w^*))}
    \Big(
    1 + \log(2Tp/\zeta)
    \Big)
    } \ge 1 - \zeta \enspace,
  \end{align}
  which is the desired result.

\end{proof}



